Probabilities Are Not Enough: Formal Controller Synthesis for Stochastic Dynamical Models with Epistemic Uncertainty

Capturing uncertainty in models of complex dynamical systems is crucial to designing safe controllers. Stochastic noise causes aleatoric uncertainty, whereas imprecise knowledge of model parameters leads to epistemic uncertainty. Several approaches use formal abstractions to synthesize policies that satisfy temporal specifications related to safety and reachability. However, the underlying models exclusively capture aleatoric but not epistemic uncertainty, and thus require that model parameters are known precisely. Our contribution to overcoming this restriction is a novel abstraction-based controller synthesis method for continuous-state models with stochastic noise and uncertain parameters. By sampling techniques and robust analysis, we capture both aleatoric and epistemic uncertainty, with a user-specified confidence level, in the transition probability intervals of a so-called interval Markov decision process (iMDP). We synthesize an optimal policy on this iMDP, which translates (with the specified confidence level) to a feedback controller for the continuous model with the same performance guarantees. Our experimental benchmarks confirm that accounting for epistemic uncertainty leads to controllers that are more robust against variations in parameter values.

==> Figures/Results/Oscillator/mass/uncertain_mass.tex <==
    \footnotesize\begin{tikzpicture}
      \begin{axis}[
          width=0.98\linewidth,
          height=3.7cm,
          ymajorgrids,
          grid style={dashed,gray!30},
          xlabel={True system parameter},
          ylabel={\% safe controllers},
          x label style={at={(axis description cs:0.5,-0.20)}},
          y label style={at={(axis description cs:-0.12,0.43)}},
          x tick label style={align=center, yshift=-0.06cm},
          xmin = 0,
          xmax = 2,
          ymin=0.60,
          ymax=1,
          xtick={0,1,2},
          %xticklabels={$m=1.00$\\$\zeta=0.50$,
          %             %$m=0.95$\\$\zeta=0.55$,
          %             $m=0.90$\\$\zeta=0.60$,
          %             %$m=0.85$\\$\zeta=0.65$,
          %             $m=0.80$\\$\zeta=0.70$},
		  xticklabels={$m=1.00$,
			$m=0.75$,
			$m=0.50$},
          ytick={0.6,0.8,1.0},
          yticklabels={60\%,80\%,100\%},
          every axis plot/.append style={line width=1pt},
          legend cell align={left},
          legend columns=1,
          legend style={at={(0.61,0.46)},
                        nodes={scale=0.85, transform shape},
                        anchor=north east, 
                        column sep=0ex,}
        ]
        
        \addplot[mark=*, mark size=1.3pt, color=BurntOrange] table[x=x, y=y, col sep=semicolon] {Figures/Results/Oscillator/mass/fraction_safe_parametric=True.csv};
        
        \addplot [name path=max_robust, draw=none] table[x=x, y=max, col sep=semicolon, forget plot] {Figures/Results/Oscillator/mass/fraction_safe_parametric=True_stats.csv};
        \addplot [name path=min_robust, draw=none] table[x=x, y=min, col sep=semicolon, forget plot] {Figures/Results/Oscillator/mass/fraction_safe_parametric=True_stats.csv};
        \addplot [fill=BurntOrange!30, forget plot] fill between[of=max_robust and min_robust];
        
        % \addplot[mark=*, mark size=1.3pt, color=BurntOrange, dashed] table[x=x, y=mdp_sim, col sep=semicolon] {Figures/Results/Oscillator/MDP_vs_iMDP_v3.csv};
        
        % \addplot [name path=upper_mdp_sim, draw=none] table[x=x, y=mdp_sim_error_plus, col sep=semicolon, forget plot] {Figures/Results/Oscillator/MDP_vs_iMDP_v3.csv};
        % \addplot [name path=lower_mdp_sim, draw=none] table[x=x, y=mdp_sim_error_min, col sep=semicolon, forget plot] {Figures/Results/Oscillator/MDP_vs_iMDP_v3.csv};
        % \addplot [fill=BurntOrange!50, forget plot, fill opacity=0.6] fill between[of=upper_mdp_sim and lower_mdp_sim];

        %%%%%%
        
        \addplot[mark=*, mark size=1.3pt, color=MidnightBlue] table[x=x, y=mean, col sep=semicolon] {Figures/Results/Oscillator/mass/fraction_safe_parametric=False_stats.csv};
        
        \addplot [name path=max_naive, draw=none] table[x=x, y=max, col sep=semicolon, forget plot] {Figures/Results/Oscillator/mass/fraction_safe_parametric=False_stats.csv};
        \addplot [name path=min_naive, draw=none] table[x=x, y=min, col sep=semicolon, forget plot] {Figures/Results/Oscillator/mass/fraction_safe_parametric=False_stats.csv};
        \addplot [fill=MidnightBlue!30, forget plot] fill between[of=max_naive and min_naive];
        
        % \addplot[mark=*, mark size=1.3pt, color=MidnightBlue, dashed] table[x=x, y=imdp_sim, col sep=semicolon] {Figures/Results/Oscillator/MDP_vs_iMDP_v3.csv};
        
        % \addplot [name path=upper_imdp_sim, draw=none] table[x=x, y=imdp_sim_error_plus, col sep=semicolon, forget plot] {Figures/Results/Oscillator/MDP_vs_iMDP_v3.csv};
        % \addplot [name path=lower_imdp_sim, draw=none] table[x=x, y=imdp_sim_error_min, col sep=semicolon, forget plot] {Figures/Results/Oscillator/MDP_vs_iMDP_v3.csv};
        % \addplot [fill=MidnightBlue!20, forget plot, fill opacity=1.0] fill between[of=upper_imdp_sim and lower_imdp_sim];
        
        \draw [dashed, very thick, gray] (axis cs:1,0.7) -- (axis cs:1,1.0);
        
        \node[pin={[pin distance=0.6cm, align=right]177.8:{Parameter\\robustness limit}}] at (axis cs:1,0.82) {};
        
        \legend{{With parameter uncertainty}, {Neglect param. uncertainty}}
      \end{axis}
    \end{tikzpicture}

==> Tables/temperature_control_table_part.tex <==
\begin{table}[t!]

\centering
\caption{\gls{iMDP} sizes and run times for different partitions on the temperature control problem (decoupled for one room).}

{\setlength{\tabcolsep}{4pt}

\scalebox{0.9}{
\begin{tabular}{cllll}
    \hline
    Epist.unc. & Partition & States & Transitions & Run time [s] 
    \\
    \hline
    & $15 \times 25$ & 378 & 84\,539 & 5.64
    % \\
    % & $25 \times 35$ & 878 & 308\,845 & 10.47
    \\
    & $35 \times 45$ & 1578 & 2\,103\,986 & 25.05
    % \\
    % & $50 \times 70$ & 3503 & 6\,149\,432 & 62.50
    \\
    & $70 \times 100$ & 7003 & 51\,742\,285 & 308.08
    \\
    \faIcon{check} & $15 \times 25$ & 378 & 100\,994 & 5.68
    % \\
    % \faIcon{check} & $25 \times 35$ & 878 & 463\,173 & 11.49
    \\
    \faIcon{check} & $35 \times 45$ & 1578 & 2\,932\,224 & 30.06
    % \\
    % \faIcon{check} & $50 \times 70$ & 3505 & 9\,520\,698 & 80.49
    \\
    \faIcon{check} & $70 \times 100$ & 7003 & 81\,763\,143 & 475.35
    \\
    \hline
\end{tabular}
}
}

\label{tab:temperature_control}
\end{table}





==> Tikz/backreachset.tex <==
\tikzstyle{boxsample} = [blue, fill=blue!30, fill opacity=0.4, text opacity=1]

\resizebox{.7\linewidth}{!}{%
\begin{tikzpicture}[scale=1.00] %, framed]

    \newcommand\orX{0}
    \newcommand\orY{0.3}
    \newcommand\boxW{1}

    \newcommand\uppX{6}
    \newcommand\uppY{3}
    
    \newcommand\originX{1}
    \newcommand\originY{1}
    \newcommand\targetX{4}
    \newcommand\targetY{2}
    
    \newcommand\dX{\targetX+0.5*\boxW}
    \newcommand\dY{\targetY+0.5*\boxW}
    
    \coordinate (vT1) at (\targetX-0.25*\boxW,\targetY-0.25*\boxW);
    \coordinate (vT2) at (\targetX+1.25*\boxW,\targetY-0.25*\boxW);
    \coordinate (vT3) at (\targetX+1.25*\boxW,\targetY+1.25*\boxW);
    \coordinate (vT4) at (\targetX-0.25*\boxW,\targetY+1.25*\boxW);
    
    \coordinate (vR1) at (\originX-\boxW*0.1,\originY+\boxW*0.25);
    \coordinate (vR2) at (\originX+\boxW*1,\originY-\boxW*0.5);
    \coordinate (vR3) at (\originX+\boxW*2.5,\originY-\boxW*0.5);
    \coordinate (vR4) at (\originX+\boxW*2.2,\originY+\boxW*1);
    \coordinate (vR5) at (\originX+\boxW*1.8,\originY+\boxW*2);
    \coordinate (vR6) at (\originX+\boxW*0.7,\originY+\boxW*2.75);
    \coordinate (vR7) at (\originX-\boxW*0.8,\originY+\boxW*2.75);
    \coordinate (vR8) at (\originX-\boxW*0.5,\originY+\boxW*1.25);
    
    % \node[rectangle] (10) at (\dX,\dY) {};
    
	% Draw backward reachable set
	% Starts in lower left corner
	\draw[red, fill=red!15, dashed] 
	(vR1) -- 
	(vR2) -- 
	(vR3) -- 
	(vR4) -- 
	(vR5) -- 
	(vR6) --
	node[anchor=north, pos=0.5, yshift=-0.1cm] {$\BackReach(\targetSet_\ell)$} 
	(vR7) -- 
	(vR8) -- 
	(vR1);
	
	% Draw states where action is enabled
	\draw[fill=red!30] (\originX+\boxW,\originY) -- (\originX+\boxW*2,\originY) -- (\originX+\boxW*2,\originX+\boxW) -- (\originX+\boxW,\originX+\boxW) node[anchor=north west, yshift=-0.1cm] {$s$} -- (\originX+\boxW,\originY);
	\draw[fill=red!30] (\originX,\originY+\boxW) -- (\originX+\boxW,\originY+\boxW) -- (\originX+\boxW,\originX+\boxW*2) -- (\originX,\originY+\boxW*2) node[anchor=north west] {$s'$} -- (\originX,\originY+\boxW);
	
	% Target set
	\draw[thick] 
	(vT1) -- 
	(vT2) node[anchor=south east, xshift=-0.0cm, yshift=0.0cm] {$\targetSet_\ell$} -- 
	(vT3) -- 
	(vT4) -- 
	(vT1);

    % Draw grid
    \foreach \x in {1,...,\uppX} % number of vertical lines
    {
        \draw[gray, dashed, opacity=0.5] (\x,\boxW/2) -- (\x,\uppY+\boxW/2);
    }
    \foreach \y in {1,...,\uppY} % number of vertical lines
    {
        \draw[gray, dashed, opacity=0.5] (\boxW/2,\y) -- (\uppX+\boxW/2,\y);
    }
    
    % Draw axes
    \draw[-{Latex[length=2mm,width=2mm]}] (\orX,\orY) -- (\uppX+\boxW-\orX,\orY);
    \draw[-{Latex[length=2mm,width=2mm]}] (\orX,\orY) -- (\orX,\uppY+\boxW-\orY);
    
    \draw[] (\uppX/2+\boxW/2,\orY) node[anchor=north] {$\state_{k}^{(1)}$};
    \draw[] (\orX,\uppY/2+\boxW/2) node[anchor=east] {$\state_{k}^{(2)}$};
    
    \draw[red, dotted, semithick] (vR1) -- (\targetX-0.25*\boxW,\targetY-0.25*\boxW);
    \draw[red, dotted, semithick] (vR2) -- (\targetX+1.25*\boxW,\targetY-0.25*\boxW);
    
    \draw[red, dotted, semithick] (vR3) -- (\targetX+1.25*\boxW,\targetY-0.25*\boxW);
    \draw[red, dotted, semithick] (vR4) -- (\targetX+1.25*\boxW,\targetY+1.25*\boxW);
    
    \draw[red, dotted, semithick] (vR5) -- (\targetX+1.25*\boxW,\targetY+1.25*\boxW);
    \draw[red, dotted, semithick] (vR6) -- (\targetX-0.25*\boxW,\targetY+1.25*\boxW);
    
    \draw[red, dotted, semithick] (vR7) -- (\targetX-0.25*\boxW,\targetY+1.25*\boxW);
    \draw[red, dotted, semithick] (vR8) -- (\targetX-0.25*\boxW,\targetY-0.25*\boxW);
    
    %     \draw[thick, red, -{Latex[length=2.0mm,width=2.0mm]}] (\originX+\boxW*1.5,\originY+\boxW*0.5) -- (\dX,\dY) node[pos=0.15, anchor=north, yshift=-0.05cm] {$a_l$};;
    	
    % 	\draw[thick, red, -{Latex[length=2.0mm,width=2.0mm]}] (\originX+\boxW*0.5,\originY+\boxW*1.5) -- (\dX,\dY) node[pos=0.1, anchor=south, yshift=-0.1cm] {$a_l$};
    
    \draw[boxsample] (3.85, 1.9) rectangle (3.85+0.7, 1.9+0.7) node [pos=.5] {\scriptsize $\boxSample_{i\ell}^{(1)}$};
    \draw[boxsample] (4.5, 2.7) rectangle (4.5+0.7, 2.7+0.7) node [pos=.5] {\scriptsize $\boxSample_{i\ell}^{(2)}$};
    \draw[boxsample] (5.4, 2.5) rectangle (5.4+0.7, 2.5+0.7) node [pos=.5] {\scriptsize $\boxSample_{i\ell}^{(3)}$};
    \draw[boxsample] (3.4, 3.1) rectangle (3.4+0.7, 3.1+0.7) node [pos=.5] {\scriptsize $\boxSample_{i\ell}^{(4)}$};
    \draw[boxsample] (5.5, 1.6) rectangle (5.5+0.7, 1.6+0.7) node [pos=.5] {\scriptsize $\boxSample_{i\ell}^{(5)}$};
    
\end{tikzpicture}
}

==> Tikz/introduction.tex <==
\usetikzlibrary{backgrounds}
\resizebox{.9\linewidth}{!}{%
\begin{tikzpicture}[scale=0.85] %[font=\sffamily]
    
    \node (helicopter) at (0,0) [minimum width=1.8cm] {};
    
    \node at (-0.4,0) [label=below:System] {\includegraphics[width=0.05\textwidth]{Figures/drone.png}};
    
    %{\huge\faIcon{helicopter}};
    
    \node (controller) at (-3,0) [label=below:Controller] {\huge\faIcon{gamepad}};
    
    \draw[-{Latex[length=2mm,width=2mm]}, dashed] (controller) -- (helicopter) node[pos=0.5, above, align=center] {Control\\input};
    
    \coordinate (xplus1) at (5.3, 0.5);
    \coordinate (xplus2) at (3.3, -0.3);
    
    \draw[fill=red!30, opacity=0.5] ($ (xplus1) + (0.6, 0.7)$ ) -- ++(-1,-0.2) -- ($ (xplus1) - (0.6, 0.7)$ ) -- ++(1,0.2) -- ($ (xplus1) + (0.6, 0.7)$ );
    
    \draw[fill=darkgreen!30, opacity=0.5] ($ (xplus2) + (0.6, 0.7)$ ) -- ++(-1,-0.2) -- ($ (xplus2) - (0.6, 0.7)$ ) -- ++(1,0.2) -- ($ (xplus2) + (0.6, 0.7)$ );
    
    \node (xplus1a) at ($ (xplus1) + (0.4,0.4) $) [circle, fill, inner sep=1.5pt, label=right:{$\text{\faIcon{weight-hanging}}^\text{\faIcon{minus}}$}] {};
    \node (xplus1b) at ($ (xplus1) - (0.05,0.45) $) [circle, fill, inner sep=1.5pt, label=right:{$\text{\faIcon{weight-hanging}}^\text{\faIcon{plus}}$}] {};
    
    \node (xplus2a) at ($ (xplus2) + (0.4,0.4) $) [circle, fill, inner sep=1.5pt, label=right:{$\text{\faIcon{weight-hanging}}^\text{\faIcon{minus}}$}] {};
    \node (xplus2b) at ($ (xplus2) - (0.05,0.45) $) [circle, fill, inner sep=1.5pt, label=right:{$\text{\faIcon{weight-hanging}}^\text{\faIcon{plus}}$}] {};
    
    \draw[-{Latex[length=2mm,width=2mm]}, red, bend right=90] (helicopter) to [out=30,in=180] node[midway, above, yshift=-0.1cm] {$\Prob\big\{$ \faIcon{wind} = high $\big\}$} (xplus1);
    \draw[-{Latex[length=2mm,width=2mm]}, darkgreen, bend right=90] (helicopter) to [out=30,in=180] node[midway, below, xshift=-0.2cm, yshift=-0.2cm] {$\Prob\{$ \faIcon{wind} = low $\}$} (xplus2);
    
    \draw[-{Latex[length=1mm,width=1mm]}] (xplus1) -- (xplus1a); 
    \draw[-{Latex[length=1mm,width=1mm]}] (xplus1) -- (xplus1b); 
    
    \draw[-{Latex[length=1mm,width=1mm]}] (xplus2) -- (xplus2a); 
    \draw[-{Latex[length=1mm,width=1mm]}] (xplus2) -- (xplus2b); 
\end{tikzpicture}%
}%
